Achieving Zero Constraint Violation for Constrained Reinforcement Learning via Conservative Natural Policy Gradient Primal-Dual Algorithm

We consider the problem of constrained Markov decision process (CMDP) in continuous state-actions spaces where the goal is to maximize the expected cumulative reward subject to some constraints. We propose a novel Conservative Natural Policy Gradient Primal-Dual Algorithm (C-NPG-PD) to achieve zero constraint violation while achieving state of the art convergence results for the objective value function. For general policy parametrization, we prove convergence of value function to global optimal upto an approximation error due to restricted policy class. We even improve the sample complexity of existing constrained NPG-PD algorithm \cite{Ding2020} from $\mathcal{O}(1/\epsilon^6)$ to $\mathcal{O}(1/\epsilon^4)$. To the best of our knowledge, this is the first work to establish zero constraint violation with Natural policy gradient style algorithms for infinite horizon discounted CMDPs. We demonstrate the merits of proposed algorithm via experimental evaluations.

==> app_property.tex <==
\section{Proof for Properties of the Objective Function}\label{sec_app_property}
\subsection{Proof for Lemma \ref{lem_smooth}}
\begin{proof}
	In order to show the smoothness, it is sufficient to bound  $\Vert\nabla^2_\theta f(\bm{J}^{\pi_\theta})\Vert$ and $\Vert\nabla^2_\theta f(\bm{J}_H^{\pi_\theta})\Vert$. By  Eq. \eqref{eq:gradient_simplified}, we have
	\begin{equation}
	\begin{split}
	\Vert\nabla_\theta^2 f(\bm{J}^{\pi_\theta})\Vert&=\Vert\mathbf{E}_{\tau\sim p(\tau\vert \theta)}\bigg[\sum_{t=0}^{\infty}\nabla_\theta^2\log\pi_\theta(a_t\vert s_t)\bigg(\sum_{m=1}^{M}\frac{\partial f}{\partial J_m^\pi}\big(\sum_{h=t}^{\infty}\gamma^hr_m(s_h,a_h)\big)\bigg)\bigg]\Vert\\
	&\leq \frac{MC}{(1-\gamma)}\sum_{t=0}^{\infty}\gamma^t\Vert\nabla_\theta^2\log\pi_\theta(a_t\vert s_t)\Vert\leq \frac{MCB}{(1-\gamma)^2}
	\end{split}
	\end{equation}
	where the last inequality holds by the Assumption \ref{ass_score}. The smoothness property for the truncated version $f(\bm{J}_H^{\pi_\theta})$ can be proved similarly.
\end{proof}
\subsection{Proof for Lemma \ref{lem_bound_truncated}}
\begin{proof}
	Notice that $\tilde{g}(\tau_i,\tau_j\vert \theta)$ is an unbiased estimator for $\nabla_\theta f(\bm{J}^{\pi_\theta})$. Moreover, $\tilde{g}(\tau_i^H,\tau_j^H)$ is an unbiased estimator for $\nabla_\theta f(\bm{J}_H^{\pi_\theta})$. Thus,
	\begin{equation}
		\begin{split}
		\Vert\nabla_\theta f(\bm{J}^{\pi_\theta})-\nabla_\theta f(\bm{J}_H^{\pi_\theta})\Vert&\overset{(a)}=\Vert\mathbf{E}[\tilde{g}(\tau_i,\tau_j\vert \theta)-\tilde{g}(\tau_i^H,\tau_j^H\vert \theta)]\Vert\leq \mathbf{E}\Vert\tilde{g}(\tau_i,\tau_j\vert \theta)-\tilde{g}(\tau_i^H,\tau_j^H\vert \theta)\Vert\\
		&\overset{(b)}\leq \mathbf{E}\Vert\tilde{g}(\tau_i,\tau_j\vert \theta)-\tilde{g}(\tau_i^H,\tau_j\vert \theta)\Vert+\mathbf{E}\Vert\tilde{g}(\tau_i^H,\tau_j\vert \theta)-\tilde{g}(\tau_i^H,\tau_j^H\vert \theta)\Vert\\
		&\overset{(c)}\leq M^{3/2}GL_f\frac{1-\gamma^H-H\gamma^H(1-\gamma)}{(1-\gamma)^3}\gamma^H+ MGC\frac{\gamma^H[1+H(1-\gamma)]}{(1-\gamma)^2}
		\end{split}
	\end{equation}
	where the step (a) and (b) hold by the triangle inequality. Step (c) holds by the Lemma \ref{lem_bound_bias2} and \ref{lem_bound_bias3}
\end{proof}	

\subsection{Proof for Lemma \ref{lem_performance_diff}}
\begin{proof}
	By the concavity of the function $f$, we have
	\begin{equation}
	\begin{aligned}
	f(\bm{J}^{\pi_\theta})&\leq  f(\bm{J}^{\pi_{\theta'}})+\nabla_{\bm{J}^{\pi_{\theta'}}} f(\bm{J}^{\pi_{\theta'}})^T(\bm{J}^{\pi_\theta}-\bm{J}^{\pi_{\theta'}})\\
	&=f(\bm{J}^{\pi_{\theta'}})+\sum_{m=1}^{M}\frac{\partial f(\bm{J}^{\pi_{\theta'}})}{\partial J_m^{\pi_{\theta'}}}(J_m^{\pi_\theta}-J_m^{\pi_{\theta'}})\\
	&=f(\bm{J}^{\pi_{\theta'}})+\sum_{m=1}^{M}\frac{\partial f(\bm{J}^{\pi_{\theta'}})}{\partial J_m^{\pi_{\theta'}}}\frac{1}{1-\gamma}\mathbf{E}_{s\sim d_\rho^{\pi_\theta}}\mathbf{E}_{a\sim\pi_\theta(\cdot\vert s)}\big[A_m^{\pi_{\theta'}}(s,a)\big]
	\end{aligned}
	\end{equation}
	where the last step comes from the policy gradient theorem \cite{sutton2000} for the standard reinforcement learning. Finally,  we get the desired result by rearranging terms.
\end{proof}
